Object Allocation Over a Network of Objects: Mobile Agents with Strict Preferences

In recent work, Gourv\`es, Lesca, and Wilczynski propose a variant of the classic housing markets model where the matching between agents and objects evolves through Pareto-improving swaps between pairs of adjacent agents in a social network. To explore the swap dynamics of their model, they pose several basic questions concerning the set of reachable matchings. In their work and other follow-up works, these questions have been studied for various classes of graphs: stars, paths, generalized stars (i.e., trees where at most one vertex has degree greater than two), trees, and cliques. For generalized stars and trees, it remains open whether a Pareto-efficient reachable matching can be found in polynomial time. In this paper, we pursue the same set of questions under a natural variant of their model. In our model, the social network is replaced by a network of objects, and a swap is allowed to take place between two agents if it is Pareto-improving and the associated objects are adjacent in the network. In those cases where the question of polynomial-time solvability versus NP-hardness has been resolved for the social network model, we are able to show that the same result holds for the network-of-objects model. In addition, for our model, we present a polynomial-time algorithm for computing a Pareto-efficient reachable matching in generalized star networks. Moreover, the object reachability algorithm that we present for path networks is significantly faster than the known polynomial-time algorithms for the same question in the social network model.

==> proof_lemma_inherit.tex <==
\begin{proof}
Let $\Agent$ denote $|\Matching|$, let $\Object$ denote
$\MaxMatched{\Matching}$, let $\Agent'$ denote $|\Matching'|$, and let
$\Object'$ denote $\MaxMatched{\Matching'}$, Since $\Matching$ belongs
to $\Decs{n}$, there exists $(\alpha,\beta)$ in
$\Encs{\Agent}{\Object}$ such that $\Matching=[\alpha,\beta]$.  Since
$\Matching'$ is contained in $\Matching$, we have $\Agent'\leq\Agent$
and $\Object'\leq\Object$.  Let $(\alpha',\beta')$ denote
$(\alpha_{1,\Agent'},\beta_{1,\Object'})$. It is straightforward to
prove that $(\alpha',\beta')$ belongs to $\Encs{\Agent'}{\Object'}$.
Hence Observation~\ref{ob:prefix} implies that
$\Matching'=[\alpha',\beta']$. We conclude that $\Matching'$ belongs
to $\Decs{n}$, as required.
\end{proof}

